Search and Rescue in a Maze-like Environment with Ant and Dijkstra Algorithms

With the growing reliability of modern Ad Hoc Networks, it is encouraging to analyze potential involvement of autonomous Ad Hoc agents in critical situations where human involvement could be perilous. One such critical scenario is the Search and Rescue effort in the event of a disaster where timely discovery and help deployment is of utmost importance. This paper demonstrates the applicability of a bio-inspired technique, namely Ant Algorithms (AA), in optimizing the search time for a near optimal path to a trapped victim, followed by the application of Dijkstra's algorithm in the rescue phase. The inherent exploratory nature of AA is put to use for a faster mapping and coverage of the unknown search space. Four different AA are implemented, with different effects of the pheromone in play. An inverted AA, with repulsive pheromones, was found to be the best fit for this particular application. After considerable exploration, upon discovery of the victim, the autonomous agents further facilitate the rescue process by forming a relay network, using the already deployed resources. Hence, the paper discusses a detailed decision making model of the swarm, segmented into two primary phases, responsible for the search and rescue respectively. Different aspects of the performance of the agent swarm are analyzed, as a function of the spatial dimensions, the complexity of the search space, the deployed search group size, and the signal permeability of the obstacles in the area.

==> Figures/alg.iAA.tex <==
%%%%%%%%%%%%%%%%%%%%
%  Begin ALGORITHM %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
initialization\;
possible moves = [stay, right, left, forward, backward]\;
\While{target not found}
{
\For{each ant}
{
Generate list of all possible next states\;
Acquire pheromone information of all next states\;
Roulette Wheel $\leftarrow$ generate probabilities of moving to each next state\;
Spin Roulette Wheel to pick next state\;
Update current position and pheromone levels\;
}
}
\caption{Basic AA Algorithm used for all decision making models, where each model differs in probability generation. The same algorithm was used to develop the AA, iAA, iAA-B, and iAA-R models by altering the equation used for probability distribution generation for the roulette wheel. }
\label{alg:iAA}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  END ALGORITHM %
%%%%%%%%%%%%%%%%%%


==> Figures/alg.iAA2.tex <==
\begin{algorithm}[h]
$Last\_Stopped$ = First agents to arrive at target\;
$Stopped\_Agents$ = [$Last\_Stopped$]\;
$Possible\_Moves$ = [right, left, forward, backward]\;

\While{Source not within $Stooped\_Agents$}
{
	\For{each agent not in $Stopped\_Agents$}
    {
    	Generate list of all possible next states\;
        Acquire pheromone information of all next states\;
        Roulette Wheel $\leftarrow$ generate probabilities of moving to each next state\;
        Spin Roulette Wheel to pick next state\;
        Update current position and pheromone levels\;
        $Agents\_Nearby$ = [All agents that could connect to $Last\_Stopped$]\;
        $Last\_Stopped$ = Min(depths of $Agents\_Nearby$)\;
        $Stopped\_Agents.push(Last\_Stopped)$;
    }
}
end function;

\caption{Algorithm to find Shortest Path to Source from Target}
\label{alg:iAA2}
\end{algorithm}

